Experiments and phenomenology of electric dipole moments

The Standard Model (SM) is the best description of fundamental particles and their interactions we have to date. From this theory, all phenomena in the macroscopic world (except for gravity) can be explained, and it has successfully predicted all outcomes of particle experiments on Earth. However, cosmological observations of the early Universe yield a large imbalance between its content of matter and antimatter, which is several orders of magnitude above the SM prediction. To explain these observations, new interactions that do not respect the charge-parity symmetry must exist beyond the SM. Such interactions would induce electric dipole moments (EDMs) in known particles. In Part I of this thesis, we propose to extend the active experimental program of EDM searches to charm and bottom baryons, $\tau$ leptons, and $\Lambda$ hyperons; also allowing the measurement of their corresponding magnetic dipole moments (MDMs). The EDM and MDM of short-lived particles can be accessed with a bent-crystal experiment to be installed in the Large Hadron Collider (LHC), while longer-lived $\Lambda$ particles can be measured at the LHCb experiment with no additional instrumentation. In Part II, an analysis of LHCb data to measure the $\Lambda$ polarization in $\Lambda_c^+ \to \Lambda \pi^+ \pi^+ \pi^-$ decays, essential ingredient for the proposed measurement, is presented. In the last part of the thesis, we derive new indirect bounds on heavy quark EDMs with already available data and explore the phenomenological implications of these and other EDM limits on New Physics models, with special emphasis on extensions of the SM with colour-octet scalars.

==> analysis/content/DTF.tex <==
% !TeX root = ../../main.tex
\newpage
\newpage





==> pheno/apppheno.tex <==

\input{pheno/appRGE}


==> pheno/diagOrderAls1.tex <==
\begin{figure}[H]
    \centering

		% TIKSET COMMON TO ALL DIAGRAMS
		\tikzset{
			    gluon/.style={decorate, draw=red,
						decoration={coil,amplitude=4pt, segment length=5pt}},
				photon/.style={decorate, draw=blue,
					decoration={snake}, draw},
				fermionin/.style={draw=black, postaction={decorate},
					decoration={markings,mark=at position .35 with {\arrow[draw=black]{>}}}},
				fermionout/.style={draw=black, postaction={decorate},
					decoration={markings,mark=at position .75 with {\arrow[draw=black]{>}}}},
				fermionprop/.style={draw=black, postaction={decorate},
					decoration={markings}},
			}
	
	\hbox{ 
	
		
		\subcaptionbox{\label{fig:als1a} $(\gamma^{(0)T})_{11}$}{
			\begin{tikzpicture}[line width=1.5 pt, node distance=2cm and 2cm ]
			
			%quark in / quark out / gluon vtx / end gluon
			\coordinate[label=below:$q $] (qi);
			\coordinate[right= 4cm of qi,label=below:$q $] (qo);
			\coordinate[right= 2cm of qi,label=below :$ $] (vg); 
			\coordinate[above= 1.5cm of vg,label=above :$ $] (eg); 	
			
			% photon vertex
			\coordinate[left=.8cm of vg,label=above :$ $] (f1); 	
			\coordinate[right= .8cm of vg,label=above :$ $] (f2); 	
			
			% labels
			\coordinate[below right=0.3cm and 0.2cm of eg,label=right :$\color{blue}{\gamma}$];
			\coordinate[below left=0.8cm and 0.1cm of f2,label=right :$\color{red}{g}$];
			
			% vertices
			\draw[fermionin] (qi) -- (vg);
			\draw[fermionout] (vg) -- (qo);
			\draw[photon] (vg) -- (eg);
			\draw[gluon] (f1) arc (-180:0:.8cm);
			
			\fill[black] (f1) circle (.1cm);
			%\fill[red] (f1) circle (.2cm);
			\fill[blue] ([xshift=-4pt,yshift=-4pt]vg) rectangle ++(8pt,8pt); %CHANGE f1/f2
			\fill[black] (f2) circle (.1cm); %CHANGE f1/f2
			
			\end{tikzpicture}
		} 
		\subcaptionbox{\label{fig:als1b} $(\gamma^{(0)T})_{22}$}{
			
			\begin{tikzpicture}[line width=1.5pt, node distance=2cm and 2cm ]
			
			%quark in / quark out / gluon vtx / end gluon
			\coordinate[label=below:$q $] (qi);
			\coordinate[right= 4cm of qi,label=below:$q $] (qo);
			\coordinate[right= 2cm of qi,label=below :$ $] (vg); 
			\coordinate[above= 1.5cm of vg,label=above :$ $] (eg); 	
			
			% photon vertex
			\coordinate[left=.8cm of vg,label=above :$ $] (f1); 	
			\coordinate[right= .8cm of vg,label=above :$ $] (f2); 	
			
			% labels
			\coordinate[below right=0.3cm and 0.2cm of eg,label=right :$\color{red}{g}$];
			\coordinate[below left=0.8cm and 0.1cm of f2,label=right :$\color{red}{g}$];
			
			% vertices
			\draw[fermionin] (qi) -- (vg);
			\draw[fermionout] (vg) -- (qo);
			\draw[gluon] (vg) -- (eg);
			\draw[gluon] (f1) arc (-180:0:.8cm);
			
			\fill[black] (f1) circle (.1cm);
			\fill[red] (vg) circle (.2cm);
			%\fill[blue] ([xshift=-4pt,yshift=-4pt]f1) rectangle ++(8pt,8pt); %CHANGE f1/f2
			\fill[black] (f2) circle (.1cm); %CHANGE f1/f2
			
			\end{tikzpicture}
		} 
			


		\subcaptionbox{\label{fig:als1c} $(\gamma^{(0)T})_{12}$}{
			\begin{tikzpicture}[line width=1.5 pt, node distance=2cm and 2cm ]
			
			%quark in / quark out / gluon vtx / end gluon
			\coordinate[label=below:$q $] (qi);
			\coordinate[right= 4cm of qi,label=below:$q $] (qo);
			\coordinate[right= 2cm of qi,label=below :$ $] (vg); 
			\coordinate[above= 1.5cm of vg,label=above :$ $] (eg); 	
			
			% photon vertex
			\coordinate[left=.8cm of vg,label=above :$ $] (f1); 	
			\coordinate[right= .8cm of vg,label=above :$ $] (f2); 	
			
			% labels
			\coordinate[below right=0.3cm and 0.2cm of eg,label=right :$\color{blue}{\gamma}$];
			\coordinate[below left=0.8cm and 0.1cm of f2,label=right :$\color{red}{g}$];
			
			% vertices
			\draw[fermionin] (qi) -- (vg);
			\draw[fermionout] (vg) -- (qo);
			\draw[photon] (vg) -- (eg);
			\draw[gluon] (f1) arc (-180:0:.8cm);
			
			\fill[black] (vg) circle (.1cm);
			\fill[red] (f1) circle (.2cm);
			%\fill[blue] ([xshift=-4pt,yshift=-4pt]vg) rectangle ++(8pt,8pt); %CHANGE f1/f2
			\fill[black] (f2) circle (.1cm); %CHANGE f1/f2
			
			\end{tikzpicture}
	    }
		
        \subcaptionbox{\label{fig:als1d} $(\gamma^{(0)T})_{21}$}{
            {\Huge ~~~~$\times$~~~        }
        }
        
	} %hbox
	
	\caption{Diagrams contributing at $\order(\als)$ to the elements of  $\gamma^{(0)}$. }	
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure}[H]
    \centering

		% TIKSET COMMON TO ALL DIAGRAMS
		\tikzset{
			    gluon/.style={decorate, draw=red,
						decoration={coil,amplitude=4pt, segment length=5pt}},
				photon/.style={decorate, draw=blue,
					decoration={snake}, draw},
				fermionin/.style={draw=black, postaction={decorate},
					decoration={markings,mark=at position .35 with {\arrow[draw=black]{>}}}},
				fermionout/.style={draw=black, postaction={decorate},
					decoration={markings,mark=at position .75 with {\arrow[draw=black]{>}}}},
				fermionprop/.style={draw=black, postaction={decorate},
					decoration={markings}},
			}
	
	\hbox{ 



		\subcaptionbox{\label{fig:als2a} $(\gamma^{(1)T})_{11}$}{
			\begin{tikzpicture}[line width=1.5 pt, node distance=2cm and 2cm ]
			
			%quark in / quark out / gluon vtx / end gluon
			\coordinate[label=below:$q $] (qi);
			\coordinate[right= 4cm of qi,label=below:$q $] (qo);
			\coordinate[right= 2cm of qi,label=below :$ $] (vg); 
			\coordinate[above= 1.5cm of vg,label=above :$ $] (eg); 	
	
	        % photon vertex
			\coordinate[left=1.4cm of vg,label=above :$ $] (f1); 	
			\coordinate[right= 1.4cm of vg,label=above :$ $] (f2); 
			
			\coordinate[left=.8cm of vg,label=above :$ $] (f3); 	
			\coordinate[right= .8cm of vg,label=above :$ $] (f4); 			
			% labels
			\coordinate[below right=0.3cm and 0.2cm of eg,label=right :$\color{blue}{\gamma}$];
			\coordinate[below left=0.8cm and 0.1cm of f2,label=right :$\color{red}{g}$];
			
			% vertices
			\draw[fermionin] (qi) -- (vg);
			\draw[fermionout] (vg) -- (qo);
			\draw[photon] (vg) -- (eg);
			\draw[gluon] (f1) arc (-180:0:1.4cm);
			\draw[gluon] (f3) arc (-180:0:0.8cm);
			
			\fill[black] (f1) circle (.1cm);
			%\fill[red] (f1) circle (.2cm);
			\fill[blue] ([xshift=-4pt,yshift=-4pt]vg) rectangle ++(8pt,8pt); %CHANGE f1/f2
			\fill[black] (f2) circle (.1cm); %CHANGE f1/f2
			\fill[black] (f3) circle (.1cm);
			\fill[black] (f4) circle (.1cm);
		
				
			\end{tikzpicture}
		} 
		
		\subcaptionbox{\label{fig:als2b} $(\gamma^{(1)T})_{22}$}{
			
			\begin{tikzpicture}[line width=1.5pt, node distance=2cm and 2cm ]
			
			%quark in / quark out / gluon vtx / end gluon
			\coordinate[label=below:$q $] (qi);
			\coordinate[right= 4cm of qi,label=below:$q $] (qo);
			\coordinate[right= 2cm of qi,label=below :$ $] (vg); 
			\coordinate[above= 1.5cm of vg,label=above :$ $] (eg); 	
			
			% photon vertex
			\coordinate[left=1.4cm of vg,label=above :$ $] (f1); 	
			\coordinate[right= 1.4cm of vg,label=above :$ $] (f2); 
			
			\coordinate[left=.8cm of vg,label=above :$ $] (f3); 	
			\coordinate[right= .8cm of vg,label=above :$ $] (f4); 			
			% labels
			\coordinate[below right=0.3cm and 0.2cm of eg,label=right :$\color{red}{g}$];
			\coordinate[below left=0.8cm and 0.1cm of f2,label=right :$\color{red}{g}$];
			
			% vertices
			\draw[fermionin] (qi) -- (vg);
			\draw[fermionout] (vg) -- (qo);
			\draw[gluon] (vg) -- (eg);
			\draw[gluon] (f1) arc (-180:0:1.4cm);
			\draw[gluon] (f3) arc (-180:0:0.8cm);
			
			\fill[black] (f1) circle (.1cm);
			\fill[red] (vg) circle (.2cm);
			%\fill[blue] ([xshift=-4pt,yshift=-4pt]f1) rectangle ++(8pt,8pt); %CHANGE f1/f2
			\fill[black] (f2) circle (.1cm); %CHANGE f1/f2
			\fill[black] (f3) circle (.1cm);
			\fill[black] (f4) circle (.1cm);
			
			\end{tikzpicture}
		} 	
		


	\subcaptionbox{\label{fig:als2c} $(\gamma^{(1)T})_{12}$}{
			
			\begin{tikzpicture}[line width=1.5pt, node distance=2cm and 2cm ]
			
			%quark in / quark out / gluon vtx / end gluon
			\coordinate[label=below:$q $] (qi);
			\coordinate[right= 4cm of qi,label=below:$q $] (qo);
			\coordinate[right= 2cm of qi,label=below :$ $] (vg); 
			\coordinate[above= 1.5cm of vg,label=above :$ $] (eg); 	
			
			% photon vertex
			\coordinate[left=1.4cm of vg,label=above :$ $] (f1); 	
			\coordinate[right= 1.4cm of vg,label=above :$ $] (f2); 
			
			\coordinate[left=.8cm of vg,label=above :$ $] (f3); 	
			\coordinate[right= .8cm of vg,label=above :$ $] (f4); 			
			% labels
			\coordinate[below right=0.3cm and 0.2cm of eg,label=right :$\color{blue}{\gamma}$];
			\coordinate[below left=0.8cm and 0.1cm of f2,label=right :$\color{red}{g}$];
			
			% vertices
			\draw[fermionin] (qi) -- (vg);
			\draw[fermionout] (vg) -- (qo);
			\draw[photon] (vg) -- (eg);
			\draw[gluon] (f1) arc (-180:0:1.4cm);
			\draw[gluon] (f3) arc (-180:0:0.8cm);
			
			\fill[black] (vg) circle (.1cm);
			\fill[red] (f1) circle (.2cm);
			%\fill[blue] ([xshift=-4pt,yshift=-4pt]f1) rectangle ++(8pt,8pt); %CHANGE f1/f2
			\fill[black] (f2) circle (.1cm); %CHANGE f1/f2
			\fill[black] (f3) circle (.1cm);
			\fill[black] (f4) circle (.1cm);
			
			\end{tikzpicture}
		}
		
    \subcaptionbox{\label{fig:als2d} $(\gamma^{(1)T})_{21}$}{
        {\Huge ~~~~$\times$~~~        }
    }		
    
	} %hbox
	
	\caption{Diagrams contributing at $\order(\als^2)$ to the elements of  $\gamma^{(1)}$. \textbf{The direct relation between $\gamma^{(1)}$ and $\Uone$ has to be shown}}	
\end{figure}


\begin{figure}[H]
    \centering

		% TIKSET COMMON TO ALL DIAGRAMS
		\tikzset{
			    gluon/.style={decorate, draw=red,
						decoration={coil,amplitude=4pt, segment length=5pt}},
				photon/.style={decorate, draw=blue,
					decoration={snake}, draw},
				fermionin/.style={draw=black, postaction={decorate},
					decoration={markings,mark=at position .35 with {\arrow[draw=black]{>}}}},
				fermionout/.style={draw=black, postaction={decorate},
					decoration={markings,mark=at position .75 with {\arrow[draw=black]{>}}}},
				fermionprop/.style={draw=black, postaction={decorate},
					decoration={markings}},
			}
	
	\hbox{ 
	
			
    \subcaptionbox{\label{fig:als3a} $(\Rqed)_{11}$}{
			
			\begin{tikzpicture}[line width=1.5pt, node distance=2cm and 2cm ]
			
			%quark in / quark out / gluon vtx / end gluon
			\coordinate[label=below:$q $] (qi);
			\coordinate[right= 4cm of qi,label=below:$q $] (qo);
			\coordinate[right= 2cm of qi,label=below :$ $] (vg); 
			\coordinate[above= 1.5cm of vg,label=above :$ $] (eg); 	
			
			% photon vertex
			\coordinate[left=.8cm of vg,label=above :$ $] (f1); 	
			\coordinate[right= .8cm of vg,label=above :$ $] (f2); 	
			
			% labels
			\coordinate[below right=0.3cm and 0.2cm of eg,label=right :$\color{blue}{\gamma}$];
			\coordinate[below left=0.8cm and 0.1cm of f2,label=right :$\color{blue}{\gamma}$];
			
			% vertices
			\draw[fermionin] (qi) -- (vg);
			\draw[fermionout] (vg) -- (qo);
			\draw[photon] (vg) -- (eg);
			\draw[photon] (f1) arc (-180:0:.8cm);
			
			\fill[black] (f1) circle (.1cm);
			%\fill[red] (vg) circle (.2cm);
			\fill[blue] ([xshift=-4pt,yshift=-4pt]vg) rectangle ++(8pt,8pt); %CHANGE f1/f2
			\fill[black] (f2) circle (.1cm); %CHANGE f1/f2
			
			\end{tikzpicture}
    }
    \subcaptionbox{\label{fig:als3b} $(\Rqed)_{22}$}{
			
			\begin{tikzpicture}[line width=1.5pt, node distance=2cm and 2cm ]
			
			%quark in / quark out / gluon vtx / end gluon
			\coordinate[label=below:$q $] (qi);
			\coordinate[right= 4cm of qi,label=below:$q $] (qo);
			\coordinate[right= 2cm of qi,label=below :$ $] (vg); 
			\coordinate[above= 1.5cm of vg,label=above :$ $] (eg); 	
			
			% photon vertex
			\coordinate[left=.8cm of vg,label=above :$ $] (f1); 	
			\coordinate[right= .8cm of vg,label=above :$ $] (f2); 	
			
			% labels
			\coordinate[below right=0.3cm and 0.2cm of eg,label=right :$\color{red}{g}$];
			\coordinate[below left=0.8cm and 0.1cm of f2,label=right :$\color{blue}{\gamma}$];
			
			% vertices
			\draw[fermionin] (qi) -- (vg);
			\draw[fermionout] (vg) -- (qo);
			\draw[gluon] (vg) -- (eg);
			\draw[photon] (f1) arc (-180:0:.8cm);
			
			\fill[black] (f1) circle (.1cm);
			\fill[red] (vg) circle (.2cm);
			%\fill[blue] ([xshift=-4pt,yshift=-4pt]f1) rectangle ++(8pt,8pt); %CHANGE f1/f2
			\fill[black] (f2) circle (.1cm); %CHANGE f1/f2
			
			\end{tikzpicture}
	}
		
    \subcaptionbox{\label{fig:als3c} $(\Rqed)_{12}$}{
        {\Huge ~~~~$\times$~~~        }
	}
	
		\subcaptionbox{\label{fig:als3d} $(\Rqed)_{21}$ (\textbf{ours})}{
			
			\begin{tikzpicture}[line width=1.5pt, node distance=2cm and 2cm ]
			
			%quark in / quark out / gluon vtx / end gluon
			\coordinate[label=below:$q $] (qi);
			\coordinate[right= 4cm of qi,label=below:$q $] (qo);
			\coordinate[right= 2cm of qi,label=below :$ $] (vg); 
			\coordinate[above= 1.5cm of vg,label=above :$ $] (eg); 	
			
			% photon vertex
			\coordinate[left=.8cm of vg,label=above :$ $] (f1); 	
			\coordinate[right= .8cm of vg,label=above :$ $] (f2); 	
			
			% labels
			\coordinate[below right=0.3cm and 0.2cm of eg,label=right :$\color{red}{g}$];
			\coordinate[below left=0.8cm and 0.1cm of f2,label=right :$\color{blue}{\gamma}$];
			
			% vertices
			\draw[fermionin] (qi) -- (vg);
			\draw[fermionout] (vg) -- (qo);
			\draw[gluon] (vg) -- (eg);
			\draw[photon] (f1) arc (-180:0:.8cm);
			
			\fill[black] (vg) circle (.1cm);
			%\fill[red] (vg) circle (.2cm);
			\fill[blue] ([xshift=-4pt,yshift=-4pt]f1) rectangle ++(8pt,8pt); %CHANGE f1/f2
			\fill[black] (f2) circle (.1cm); %CHANGE f1/f2
			
			\end{tikzpicture}
		} 



	} %hbox
	
	\caption{Diagrams contributing at $\order(\ale)$ to the elements of  $\gamma^{(2)}$. }	
\end{figure}

==> pheno/diagramsEDMsMW.tex <==
\newcommand{\labl}[1]{%
	\ifthenelse{\equal{gluon}{#1}}{${\color{red}g}$}{}%
	\ifthenelse{\equal{photon}{#1}}{${\color{blue}\gamma}$}{}%
	\ifthenelse{\equal{fermion}{#1}}{$f$}{}%
	\ifthenelse{\equal{W+}{#1}}{$W^{\pm}$}{}%
	\ifthenelse{\equal{Z}{#1}}{$Z$}{}%
	\ifthenelse{\equal{S+}{#1}}{$S^{\pm}$}{}%
	\ifthenelse{\equal{S0}{#1}}{$S^{0}_{R,I}$}{}%
	\ifthenelse{\equal{S0R}{#1}}{$S^{0}_{R}$}{}%
	\ifthenelse{\equal{S0I}{#1}}{$S^{0}_{I}$}{}%
	
	\ifthenelse{\equal{t}{#1}}{$t$}{}%
	\ifthenelse{\equal{b}{#1}}{$b$}{}%
	\ifthenelse{\equal{q}{#1}}{$q$}{}%
	\ifthenelse{\equal{qprime}{#1}}{$q^\prime$}{}%
	
	\ifthenelse{\equal{bthreshold}{#1}}{$b$}{}%
	\ifthenelse{\equal{cthreshold}{#1}}{$c$}{}%
	
	\ifthenelse{\equal{H0}{#1}}{$H^{0}$}{}%
	
}

\newcommand{\dlabl}[1]{%
	\ifthenelse{\equal{bthreshold}{#1}}{$\tilde{d}_b$}{}%
	\ifthenelse{\equal{cthreshold}{#1}}{$\tilde{d}_c$}{}%
}

% TIKSET COMMON TO ALL DIAGRAMS
\tikzset{
	gluon/.style={decorate, draw=red,
		decoration={coil,amplitude=4pt, segment length=5pt}},
	photon/.style={decorate, draw=blue,
		decoration={snake}, draw},
	fermionin/.style={draw=black, postaction={decorate},
		decoration={markings,mark=at position .35 with {\arrow[draw=black]{>}}}},
	fermionout/.style={draw=black, postaction={decorate},
		decoration={markings,mark=at position .75 with {\arrow[draw=black]{>}}}},
	fermionprop/.style={draw=black, postaction={decorate},
		decoration={markings}},
	fermion/.style={draw=black, postaction={decorate},
		decoration={markings,mark=at position .5 with {\arrow[draw=black]{>}}}},
	W+/.style={decorate, draw=black, decoration={snake}, draw},
	Z/.style={decorate, draw=black, decoration={snake}, draw},
	S+/.style={decorate, draw=black, dashed, draw},
	S0/.style={decorate, draw=black, dashed, draw},
	S0R/.style={decorate, draw=black, dashed, draw},
	S0I/.style={decorate, draw=black, dashed, draw},
	t/.style={draw=black, postaction={decorate},
		decoration={markings,mark=at position .65 with {\arrow[draw=black]{>}}}},
	b/.style={draw=black, postaction={decorate},
		decoration={markings,mark=at position .65 with {\arrow[draw=black]{>}}}},
	q/.style={draw=black, postaction={decorate},
		decoration={markings,mark=at position .65 with {\arrow[draw=black]{>}}}},
    qprime/.style={draw=black, postaction={decorate},
		decoration={markings,mark=at position .65 with {\arrow[draw=black]{>}}}},
	bthreshold/.style={draw=black, postaction={decorate},
		decoration={markings,mark=at position .33 with {\arrow[draw=black]{>}}}},
	cthreshold/.style={draw=black, postaction={decorate},
		decoration={markings,mark=at position .33 with {\arrow[draw=black]{>}}}},
	H0/.style={decorate, draw=black, dashed, draw}
}
	
\newcommand{\barzee}[4]{

	\leavevmode	
	\hbox{		
		\begin{tikzpicture}[line width=1.5 pt, node distance=2cm and 2cm ]
		
		%quark in / quark out / gluon vtx / end gluon
		\coordinate[label=below:$q $] (qi);
		\coordinate[right= 4cm of qi,label=below:$q $] (qo);
		
		\coordinate[right=1.1cm of qi,label=above :$ $] (f1); 	
		\coordinate[left= 1.1cm of qo,label=above :$ $] (f2); 
		%circle
		\coordinate[above right = 1.4cm and 2 cm of qi,label=left :$  $] (c); 
		\coordinate[right = 0.7cm of c,label=above : $ $ ] (rc); 
		\coordinate[left = 0.7cm of c,label=above : $ $ ] (lc); 
		\coordinate[below left= 0.5cm and 0.5cm of c,label=below:$ $] (t1);
		\coordinate[below right= 0.5cm and 0.5cm of c,label=below:$ $] (t2); 
		\coordinate[above= 0.7cm of c,label=below :$  $] (vp); 
		
		\coordinate[above= 0.7cm of vp,label=right : \labl{#4} ] (ep); 	
		
		% labels
		\coordinate[below left = 0.35 and 0.3 of t1,label=left:\labl{#1}];
		\coordinate[below right = 0.35 and 0.3 of t2,label=right: \labl{#2} ];
		\coordinate[above left = 0.4cm and 0.0cm of rc,label=right : \labl{#3} ]; 
		
		% vertices
		\draw[fermionin] (qi) -- (f1);
		\draw[fermionprop] (f1) -- (f2);
		\draw[fermionout] (f2) -- (qo);
		
		\draw[#2] (t2) -- (f2);
		\draw[#1] (f1) -- (t1);
		\draw[#4] (vp) -- (ep);
		
		\draw[#3] (lc) arc (180:540:0.7cm);
		
		\fill[black] (f1) circle (.1cm);
		\fill[black] (f2) circle (.1cm);
	
        %add some verticle space
        \coordinate[above=0.5cm of ep,label=below :~]; 	
        \coordinate[below=0.5cm of f1,label=below :~]; 	
	        
		\end{tikzpicture}
		
	}  
}




\newcommand{\barzeeFC}[5]{

	\leavevmode	
	\hbox{		
		\begin{tikzpicture}[line width=1.5 pt, node distance=2cm and 2cm ]
		
		%quark in / quark out / gluon vtx / end gluon
		\coordinate[label=below:$q $] (qi);
		\coordinate[right= 4cm of qi,label=below:$q $] (qo);
		
		\coordinate[right=1.1cm of qi,label=above :$ $] (f1); 	
		\coordinate[left= 1.1cm of qo,label=above :$ $] (f2); 
		%circle
		\coordinate[above right = 1.4cm and 2 cm of qi,label=left :$  $] (c); 
		\coordinate[right = 0.7cm of c,label=above : $ $ ] (rc); 
		\coordinate[below left= 0.5cm and 0.5cm of c,label=below:$ $] (t1);
		\coordinate[below right= 0.5cm and 0.5cm of c,label=below:$ $] (t2); 
		\coordinate[above= 0.7cm of c,label=below :$  $] (vp); 
		
		\coordinate[above= 0.7cm of vp,label=right : \labl{#4} ] (ep); 	
		
		% labels
		\coordinate[below left = 0.35 and 0.3 of t1,label=left:\labl{#1}];
		\coordinate[below right = 0.35 and 0.3 of t2,label=right: \labl{#2} ];
 		\coordinate[above= 0.4cm of rc,label=right : \labl{#3} ];
		\coordinate[below = 0.7cm of c,label=below: \labl{#5} ]; 
		
		% vertices
		\draw[fermionin] (qi) -- (f1);
		\draw[fermionprop] (f1) -- (f2);
		\draw[fermionout] (f2) -- (qo);
		
		\draw[#2] (t2) -- (f2);
		\draw[#1] (f1) -- (t1);
		\draw[#4] (vp) -- (ep);
		
 		\draw[#3] (t2) arc (-45:225:0.7cm);
		
		\draw[#5] (t1) arc (225:315:0.7cm);
		
		\fill[black] (f1) circle (.1cm);
		\fill[black] (f2) circle (.1cm);
	
        %add some verticle space
        \coordinate[above=0.5cm of ep,label=below :~]; 	
        \coordinate[below=0.5cm of f1,label=below :~]; 	
	        
		\end{tikzpicture}
		
	}  
}


\newcommand{\weinberg}[3]{

\leavevmode
\hbox{
    \begin{tikzpicture}[line width=1.5 pt, node distance=2cm and 2cm ]
			
            %center
			\coordinate[] (c);

			%touching gluon points
			\coordinate[left= 1cm of c, label=right:$  $] (gt1);
			\coordinate[above right = 0.71cm and 0.71cm of c,label=below:$ $] (gt2);
			\coordinate[below right = 0.71cm and 0.71cm of c,label=below:$ $] (gt3); 	
			
			%out gluon points
			\coordinate[left= 2cm of c, label=below:$  $] (go1);
			\coordinate[above right = 1.42cm and 1.42cm of c,label=right:$ $] (go2);
			\coordinate[below right = 1.42cm and 1.42cm of c,label=below:$ $] (go3); 	
			
			%touching points inner propagator 
			\coordinate[above= 1cm of c, label=below:$  $] (vu);
			\coordinate[below= 1cm of c, label=below:$  $] (vd);
		
 			% labels
 			\coordinate[below left=0.25 and 0.8 of vu,label=above :\labl{#1}];
 			\coordinate[below right=0.8 and 0.6 of gt2,label=above :\labl{#3}];
			\coordinate[left = 0.05 of c, label=left:\labl{#2}];
			
			
			% vertices
			\draw[#1] (vd) arc (-90:-270:1.0cm);
			\draw[#3] (vu) arc (90:-90:1.0cm);
			\draw[#2] (vd) -- (vu);
			
			\draw[gluon] (go1) -- (gt1);
			\draw[gluon] (gt2) -- (go2);
			\draw[gluon] (gt3) -- (go3);

			\fill[black] (vu) circle (.1cm);
			\fill[black] (vd) circle (.1cm);
	
	       % %add some verticle space
	       \coordinate[above=1.5cm of c,label=below :~]; 	
	       \coordinate[below=1.5cm of c,label=below :~]; 	
	        
			\end{tikzpicture} 

    }

}


\newcommand{\weinbergBuble}[3]{

\leavevmode
\hbox{
    \begin{tikzpicture}[line width=1.5 pt, node distance=2cm and 2cm ]
			
            %center
			\coordinate[] (c);

			%touching gluon points
			\coordinate[left= 1cm of c, label=right:$  $] (gt1);
			\coordinate[above right = 0.71cm and 0.71cm of c,label=below:$ $] (gt2);
			\coordinate[below right = 0.71cm and 0.71cm of c,label=below:$ $] (gt3); 	
			
			%out gluon points
			\coordinate[left= 2cm of c, label=below:$  $] (go1);
			\coordinate[above right = 1.42cm and 1.42cm of c,label=right:$ $] (go2);
			\coordinate[below right = 1.42cm and 1.42cm of c,label=below:$ $] (go3); 	
			
			%touching points inner propagator 
			\coordinate[above= 1cm of c, label=below:$  $] (vu);
			\coordinate[above left= 0.5cm and 0.866cm of c, label=below:$  $] (vd);
		
 			% labels
 			\coordinate[below left=0.25 and 0.8 of vu,label=above :\labl{#3}];
 			\coordinate[below right=0.8 and 0.6 of gt2,label=above :\labl{#1}];
			\coordinate[below left = 0.05 and 0.05 of c, label=left:\labl{#2}];
			
			
			% vertices
			\draw[#1] (vu) arc (90:-210:1.0cm);
		    \draw[#2] (vu) arc (30:-150:0.5cm);
		    \draw[#3] (vd) arc (150:90:1.0cm);
			
			\draw[gluon] (go1) -- (gt1);
			\draw[gluon] (gt2) -- (go2);
			\draw[gluon] (gt3) -- (go3);

			\fill[black] (vu) circle (.1cm);
			\fill[black] (vd) circle (.1cm);

	       % %add some verticle space
	       \coordinate[above=1.5cm of c,label=below :~]; 	
	       \coordinate[below=1.5cm of c,label=below :~]; 	
	        
			\end{tikzpicture} 

    }

}





\newcommand{\weinbergOneLoop}[1]{
	
	\leavevmode
	\hbox{
		\begin{tikzpicture}[line width=1.5 pt, node distance=2cm and 2cm ]
		
		%center
		\coordinate[] (c);
		
		%touching gluon points
		\coordinate[left= 1cm of c, label=right:$  $] (gt1);
		\coordinate[above right = 0.71cm and 0.71cm of c,label=below:$ $] (gt2);
		\coordinate[below right = 0.71cm and 0.71cm of c,label=below:$ $] (gt3); 	
		
		%out gluon points
		\coordinate[left= 2cm of c, label=below:$  $] (go1);
		\coordinate[above right = 1.42cm and 1.42cm of c,label=right:$ $] (go2);
		\coordinate[below right = 1.42cm and 1.42cm of c,label=below:$ $] (go3); 	
		
		%touching points inner propagator 
		\coordinate[above= 1cm of c, label=below:$  $] (vu);
		\coordinate[above left= 0.5cm and 0.866cm of c, label=below:$  $] (vd);
		
		% labels
		\coordinate[below right=0.8 and 0.6 of gt2,label=above :\labl{#1}];
% 		\coordinate[below left=0.25 and 0.8 of vu,label=above :\labl{#1}];
		\coordinate[above left=0.4 and 0.2 of gt1,label=above :\dlabl{#1}];
		
		
		% vertices
		\draw[#1] (vu) arc (90:-270:1.0cm);
		
		\draw[gluon] (go1) -- (gt1);
		\draw[gluon] (gt2) -- (go2);
		\draw[gluon] (gt3) -- (go3);
		
		\fill[red] (gt1) circle (.25cm);
		
	       % %add some verticle space
	       \coordinate[above=1.5cm of c,label=below :~]; 	
	       \coordinate[below=1.5cm of c,label=below :~]; 	
	        	
		\end{tikzpicture} 
		
	}
	
}





\newcommand{\oneloop}[4]{

\leavevmode

\hbox{
		 \begin{tikzpicture}[line width=1.5 pt,scale=0.95, every node/.style={transform shape} ]
			
			%quark in / quark out / gluon vtx / end gluon
			\coordinate[label=below:\labl{#1}] (qi);
			\coordinate[right= 4cm of qi,label=below:\labl{#1}] (qo);

			\coordinate[right=1.1cm of qi,label=above :] (f1); 	
			\coordinate[left= 1.1cm of qo,label=above :$ $] (f2); 			
			
			\coordinate[above right= 1.3cm and 0.9cm of f1,label=below :$ $] (vp); 
			\coordinate[above= 1.0cm of vp,label=right : \labl{#4} ] (ep); 	
		
 			% labels
 			\coordinate[below =1.3 of vp,label=below: \labl{#3}];
 			\coordinate[below left=0.5cm and 0.5cm of vp,label=left: \labl{#2} ];
 			\coordinate[below right=0.5cm and 0.5cm of vp,label=right: $ $];
 			
			% vertices
			\draw[#1] (qi) -- (f1);
			\draw[#1] (f2) -- (qo);
			\draw[#2] (f1) -- (vp);
			\draw[#2] (vp) -- (f2);
			\draw[#4] (vp) -- (ep);
			\draw[#3] (f1) -- (f2);
			
			\fill[black] (f1) circle (.1cm);
			\fill[black] (f2) circle (.1cm);
			\fill[black] (vp) circle (.1cm);

	       % %add some verticle space
	       \coordinate[above=0.5cm of ep,label=below :~]; 	
	       \coordinate[below=0.5cm of qi,label=below :~]; 	
	        	
			\end{tikzpicture}
			
    }

}





\newcommand{\triangleDiag}[6]{

\leavevmode

\hbox{


\begin{tikzpicture}[line width=1.5 pt,node distance=1 cm and 1.5 cm]
\coordinate[] (aux);
\coordinate[below = 1.6 cm of aux] (aux2);
\coordinate[below = 0.8 cm of aux, label = right: \labl{#4}] (auxaux);
\coordinate[left = 0.5 cm of aux, label =  left: \labl{#5}];
\coordinate[left = 0.5 cm of aux2, label =  left: \labl{#6}];
\coordinate[ right = of aux, label= above :\labl{#2}] (g1);
\coordinate[ right = of aux2, label= below :\labl{#3}] (g2);
\coordinate[left = of auxaux] (aux3);
\coordinate[ left = of aux3, label = above:\labl{#1}] (h);
\draw[#2] (g1) -- (aux);
\draw[#3] (g2) -- (aux2);
\draw[#4] (aux2) -- (aux);
\draw[#5] (aux) -- (aux3);
\draw[#6] (aux3) -- (aux2);
\draw[#1] (aux3) -- (h);
\draw[fill=black] (aux) circle (.03cm);
\draw[fill=black] (aux2) circle (.03cm);
\draw[fill=black] (aux3) circle (.03cm);
\end{tikzpicture}

}
}



\newcommand{\weinbergOneLoopQQGG}[1]{
	
	\leavevmode
	\hbox{
		\begin{tikzpicture}[line width=1.5 pt, node distance=2cm and 2cm ]
		
		%center
		\coordinate[] (c);
		
		%touching gluon points
		\coordinate[left= 1cm of c, label=right:$  $] (gt1);
		\coordinate[right= 1cm of c, label=below:$ $] (gt2);
		\coordinate[right= 1cm of c, label=below:$ $] (gt3); 	
		
		%out gluon points
		\coordinate[left= 2cm of c, label=below:$  $] (go1);
		\coordinate[above right = 1.1cm and 1.9cm of c,label=right:$ $] (go2);
		\coordinate[below right = 1.1cm and 1.9cm of c,label=below:$ $] (go3); 	
		
		%touching points inner propagator 
		\coordinate[above= 1cm of c, label=below:$  $] (vu);
		\coordinate[below= 1cm of c, label=below:$  $] (vd);
		
		% labels
		\coordinate[below left=0.25 and 0.8 of vu,label=above :\labl{#1}];
		
		% vertices
		\draw[#1] (vd) arc (-90:-450:1.0cm);
		
		\draw[gluon] (go1) -- (gt1);
		\draw[gluon] (gt2) -- (go2);
		\draw[gluon] (gt3) -- (go3);
		
		\fill[red] (gt2) circle (.25cm);
		
	       % %add some verticle space
	       \coordinate[above=1.5cm of c,label=below :~]; 	
	       \coordinate[below=1.5cm of c,label=below :~]; 	
	        
		\end{tikzpicture} 
		
	}
	
}





\newcommand{\fourFermionNeutral}[5]{
	
	\leavevmode
	\hbox{
		\begin{tikzpicture}[line width=1.5 pt, node distance=2cm and 2cm ]
		
		%center
		\coordinate[] (c);
		
		%two vertices
		\coordinate[left= 1cm of c, label=right:$  $] (vl);
		\coordinate[right= 1cm of c, label=below:$ $] (vr);
		
		%out fermion points
		\coordinate[above left= 1.5cm and 1.5cm of vl, label=below:$  $] (q1);
		\coordinate[below left= 1.5cm and 1.5cm of vl, label=below:$  $] (q2);
		\coordinate[above right= 1.5cm and 1.5cm of vr, label=below:$  $] (q3);
		\coordinate[below right= 1.5cm and 1.5cm of vr, label=below:$  $] (q4);
		
	
		% labels
		\coordinate[below=0.25cm of c,label=below :\labl{#5}];
		
		\coordinate[right=0.8cm of q1,label=below :\labl{#1}];
		\coordinate[right=0.8cm of q2,label=above :\labl{#2}];
		\coordinate[left=0.8cm of q3,label=below :\labl{#3}];
		\coordinate[left=0.8cm of q4,label=above :\labl{#4}];
		
% 		% vertices

		\draw[#1] (q1) -- (vl);
		\draw[#2] (vl) -- (q2);
		\draw[#3] (q3) -- (vr);
		\draw[#4] (vr) -- (q4);
		\draw[#5] (vl) -- (vr);
		
		\fill[black] (vl) circle (.1cm);
		\fill[black] (vr) circle (.1cm);
		
	       % %add some verticle space
	       \coordinate[above=1.5cm of c,label=below :~]; 	
	       \coordinate[below=1.5cm of c,label=below :~]; 	
	        
		\end{tikzpicture} 
		
	}
	
}













\newcommand{\mpdiag}[2]{
\hspace*{-0.5cm}\begin{minipage}[c]{0.36\textwidth}
    #1
\end{minipage}
\begin{minipage}[c]{0.61\textwidth}
    #2
\end{minipage}
}




\newcommand{\weinbergMomenta}{

\leavevmode

\hbox{
    \begin{tikzpicture}[line width=1.5 pt, node distance=2cm and 2cm ]
			
            %center
			\coordinate[] (c);

			%touching gluon points
			\coordinate[left= 1.5cm of c, label=right:$  $] (gt1);
			\coordinate[above right = 1.06cm and 1.06cm of c,label=below:$ $] (gt2);
			\coordinate[below right = 1.06cm and 1.06cm of c,label=below:$ $] (gt3); 	
			
			%out gluon points
			\coordinate[left= 3cm of c, label=below:$  $] (go1);
			\coordinate[above right = 2.13cm and 2.13cm of c,label=right:$ $] (go2);
			\coordinate[below right = 2.13cm and 2.13cm of c,label=below:$ $] (go3); 	
			
			%touching points inner propagator 
			\coordinate[above= 1.5cm of c, label=below:$  $] (vu);
			\coordinate[below= 1.5cm of c, label=below:$  $] (vd);
		
 			% labels particles
 			\coordinate[below left=0.25 and 0.8 of vu,label=above :\labl{t}];
 			\coordinate[below right=0.8 and 0.6 of gt2,label=above :$ $];
			\coordinate[above right = 0.8 and -0.1 of c, label=right:\labl{S0}];
			
			% momenta arrows
			\coordinate[above right=0.4cm and 0.2cm of go1,label=right :{\rotatebox{180}{$\longrightarrow$}}];
			\coordinate[below left=0.8cm and 0.6cm of go2,label=right :{\rotatebox{225}{$\longrightarrow$}}];
			\coordinate[above left=0.8cm and 0.6cm of go3,label=right :{\rotatebox{135}{$\longrightarrow$}}];
			\coordinate[left= 0.0cm of c,label=left :{\rotatebox{270}{$\longrightarrow$}}];
			
			% momenta labels
			\coordinate[above right=0.8cm and 0.2cm of go1,label=right :$ p_3 $];
			\coordinate[below left=1.1cm and 0.2cm of go2,label=right :$p_1$];
			\coordinate[above left=1.1cm and 0.2cm of go3,label=right :$p_2$];
			\coordinate[right= 1.5cm of c,label=left :$ k_1 + k_2$];

			% index
			\coordinate[left=0.8cm of go1,label=right :$\mu_3$];
			\coordinate[right=0.2cm of go2,label=right :$\mu_1$];
			\coordinate[right=0.2cm of go3,label=right :$\mu_2$];

			% vertices
			\draw[t] (vd) arc (-90:-270:1.5cm);
			\draw[t] (vu) arc (90:-90:1.5cm);
			\draw[S0] (vd) -- (vu);
			
			\draw[gluon] (go1) -- (gt1);
			\draw[gluon] (gt2) -- (go2);
			\draw[gluon] (gt3) -- (go3);

			\fill[black] (vu) circle (.1cm);
			\fill[black] (vd) circle (.1cm);
	
	       % %add some verticle space
	       % \coordinate[above=0.8cm of vu,label=below :~]; 	
	       % \coordinate[below=0.8cm of vd,label=below :~]; 	
	        
			\end{tikzpicture} 

    }

}

% Barr-Zee diagram with form factor as vertex
\newcommand{\barzeeEffectivegg}{
	
	\leavevmode	
	\hbox{		
		\begin{tikzpicture}[line width=1.5 pt, node distance=2cm and 2cm ]
		
		%quark in / quark out / gluon vtx / end gluon
		\coordinate[label=below:$q $] (qi);
		\coordinate[right= 4cm of qi,label=below:$q $] (qo);
		
		\coordinate[right=1.1cm of qi,label=above :$ $] (f1); 	
		\coordinate[left= 1.1cm of qo,label=above :$ $] (f2); 
		%circle
		\coordinate[above right = 1.4cm and 2 cm of qi,label=left :$  $] (c); 
		\coordinate[above = 0.15cm of c,label=left :$  $] (cup);
		\coordinate[below = 0.1cm of c,label=left :$  $] (cdown);  
		\coordinate[above= 1.2cm of c,label=right : \labl{gluon} ] (ep); 	
		
		% labels
		\coordinate[above right = 0.7 and 0.3 of f1,label=left:\labl{S0}];
		\coordinate[above left = 0.7 and 0.3 of f2,label=right: \labl{gluon} ];
		\coordinate[above right = 0.1 and 0.3 of c,label=right: $i\Gamma^{\mu\nu}_g$ ];
	
		% vertices
		\draw[fermionin] (qi) -- (f1);
		\draw[fermionprop] (f1) -- (f2);
		\draw[fermionout] (f2) -- (qo);
		
		\draw[gluon] (c) -- (f2);
		\draw[S0] (f1) -- (c);
		\draw[gluon] (cup) -- (ep);
		
		
		\draw[fill=gray] (cdown) circle (.3cm);
		\fill[black] (f1) circle (.1cm);
		\fill[black] (f2) circle (.1cm);
		
		%add some verticle space
		\coordinate[above=0.5cm of ep,label=below :~]; 	
		\coordinate[below=0.5cm of f1,label=below :~]; 	
		
		\end{tikzpicture}
		
	}  
}

\newcommand{\barzeeEffectivephg}{
	
	\leavevmode	
	\hbox{		
		\begin{tikzpicture}[line width=1.5 pt, node distance=2cm and 2cm ]
		
		%quark in / quark out / gluon vtx / end gluon
		\coordinate[label=below:$q $] (qi);
		\coordinate[right= 4cm of qi,label=below:$q $] (qo);
		
		\coordinate[right=1.1cm of qi,label=above :$ $] (f1); 	
		\coordinate[left= 1.1cm of qo,label=above :$ $] (f2); 
		%circle
		\coordinate[above right = 1.4cm and 2 cm of qi,label=left :$  $] (c); 
		\coordinate[above = 0.15cm of c,label=left :$  $] (cup);
		\coordinate[below = 0.1cm of c,label=left :$  $] (cdown);  
		\coordinate[above= 1.2cm of c,label=right : \labl{photon} ] (ep); 	
		
		% labels
		\coordinate[above right = 0.7 and 0.3 of f1,label=left:\labl{S0}];
		\coordinate[above left = 0.7 and 0.3 of f2,label=right: \labl{gluon} ];
		\coordinate[above right = 0.1 and 0.3 of c,label=right: $i\Gamma^{\mu\nu}_\gamma$ ];
		
		% vertices
		\draw[fermionin] (qi) -- (f1);
		\draw[fermionprop] (f1) -- (f2);
		\draw[fermionout] (f2) -- (qo);
		
		\draw[gluon] (c) -- (f2);
		\draw[S0] (f1) -- (c);
		\draw[photon] (cup) -- (ep);
		
		
		\draw[fill=gray] (cdown) circle (.3cm);
		\fill[black] (f1) circle (.1cm);
		\fill[black] (f2) circle (.1cm);
		
		%add some verticle space
		\coordinate[above=0.5cm of ep,label=below :~]; 	
		\coordinate[below=0.5cm of f1,label=below :~]; 	
		
		\end{tikzpicture}
		
	}  
}

\newcommand{\effVertexgph}{
	
	\leavevmode	
	\hbox{		
		
		\begin{tikzpicture}[line width=1.5 pt,node distance=1 cm and 1.5 cm]
		\coordinate[] (aux);
		\coordinate[ above right  = of aux, label= above :$  \vec{q} {,}  \, \mu  $] (g1);
		\coordinate[ above right  = of aux, label= right :$ \gamma  $] (g1);
		\coordinate[ below right  = of aux, label= below :$  \vec{k} {,}  \,\nu {,} \, b$] (g2);
		\coordinate[ below right  = of aux, label= right :$ g^*$] (g2);
		\coordinate[ left = 2 cm of aux, label = above:$S_{R,I}^*  $] (h);
		\coordinate[ left = 2 cm of aux, label = below:$  (\vec{k}-\vec{q})  {,} \, a$] (h);
		\draw[photon] (g1) -- (aux);
		%\draw[gluon] (g2) -- (aux);
		\draw[gluon] (g2) -- (aux);
		\draw[S0] (aux) -- (h);
		\draw[fill=gray] (aux) circle (.3cm);
		\end{tikzpicture}
		
	}  
}

\newcommand{\effVertexgg}{
	
	\leavevmode	
	\hbox{		
		
		\begin{tikzpicture}[line width=1.5 pt,node distance=1 cm and 1.5 cm]
		\coordinate[] (aux);
		\coordinate[ above right  = of aux, label= above :$  \vec{q} {,}  \, \mu {,}  \, b$] (g1);
		\coordinate[ above right  = of aux, label= right :$ g $] (g1);
		\coordinate[ below right  = of aux, label= below :$  \vec{k} {,}  \,\nu{,}  \, c$] (g2);
		\coordinate[ below right  = of aux, label= right :$ g^* $] (g2);
		\coordinate[ left = 2 cm of aux, label = above:$S_{R,I}^*  $] (h);
		\coordinate[ left = 2 cm of aux, label = below:$  (\vec{k}-\vec{q})  {,} \, a$] (h);
		\draw[gluon] (g1) -- (aux);
		\draw[gluon] (g2) -- (aux);
		%\draw[photon] (g2) -- (aux);
		\draw[S0] (aux) -- (h);
		\draw[fill=gray] (aux) circle (.3cm);
		\end{tikzpicture}
		
	}  
}





%%% ERASE LATER: EXAMPLE OF LOOP WITH MOMENTA DIRECTIONS
\newcommand{\examplediag}{

\leavevmode

\hbox{


	\begin{tikzpicture}[line width=1.5 pt, node distance=2cm and 2cm ]
			
			%quark in / quark out / gluon vtx / end gluon
			\coordinate[label=below:$q $] (qi);
			\coordinate[right= 6cm of qi,label=below:$q $] (qo);
			\coordinate[right= 3cm of qi,label=below :$ $] (vg); 
			\coordinate[above= 2.5cm of vg,label=above :$ $] (eg); 	
			
			% photon vertex
			\coordinate[left=1.6cm of vg,label=above :$ $] (f1); 	
			\coordinate[right= 1.6cm of vg,label=above :$ $] (f2); 	
			
			% labels
			\coordinate[below right=0.3cm and 0.2cm of eg,label=right :$\color{red}{g}$];
			\coordinate[below left=1.0cm and 0.15cm of f2,label=right :$\color{blue}{\gamma}$];
			
			\coordinate[below left=1.0cm and 0.4cm of eg,label=left :$p_3$];
			\coordinate[below left=1.0cm and 0.2cm of eg,label=left :{\rotatebox{90}{$\longrightarrow$}}];
        	\coordinate[above right=0.4cm and 0.6cm of qi,label=above :{$p_1$ }];
        	\coordinate[above right=0.2cm and 0.6cm of qi,label=above :{$\longrightarrow$ }];
        	\coordinate[above left=0.4cm and 0.6cm of qo,label=above :{$p_2$ }];
        	\coordinate[above left=0.2cm and 0.6cm of qo,label=above :{$\longrightarrow$ }];
        	\coordinate[above left=0.4cm and 0.6cm of f2,label=above :{$p_2 + k$ }];
        	\coordinate[above left=0.2cm and 0.6cm of f2,label=above :{$\longrightarrow$ }];
        	\coordinate[above right=0.4cm and 0.6cm of f1,label=above :{$p_1 + k$ }];
        	\coordinate[above right=0.2cm and 0.6cm of f1,label=above :{$\longrightarrow$ }];
        	\coordinate[below right=0.8cm and 0.0cm of vg,label=below :{\LARGE \rotatebox{180}{$\curvearrowright$}}];
        	\coordinate[below right=0.4cm and 0.0cm of vg,label=below :{$k$}];
        	
        	\coordinate[above left=0.2cm and 0.2cm of eg,label=left :{$\mathfrak{X},a$}];
        	\coordinate[below left=0.4cm and 0.1cm of f1,label=left :{$\mu_1$ }];
        	\coordinate[below right=0.4cm and 0.1cm of f2,label=right :{$\mu$ }];
        	
			% vertices
			\draw[fermionin] (qi) -- (vg);
			\draw[fermionout] (vg) -- (qo);
			\draw[gluon] (vg) -- (eg);
			\draw[photon] (f1) arc (-180:0:1.6cm);
			
			\fill[black] (vg) circle (.1cm);
			\fill[blue] ([xshift=-4pt,yshift=-4pt]f1) rectangle ++(8pt,8pt); %CHANGE f1/f2
			\fill[black] (f2) circle (.1cm); %CHANGE f1/f2
			
			\end{tikzpicture}
    
}

}



